Few Shot Semantic Segmentation: a review of methodologies, benchmarks, and open challenges

Semantic segmentation, vital for applications ranging from autonomous driving to robotics, faces significant challenges in domains where collecting large annotated datasets is difficult or prohibitively expensive. In such contexts, such as medicine and agriculture, the scarcity of training images hampers progress. Introducing Few-Shot Semantic Segmentation, a novel task in computer vision, which aims at designing models capable of segmenting new semantic classes with only a few examples. This paper consists of a comprehensive survey of Few-Shot Semantic Segmentation, tracing its evolution and exploring various model designs, from the more popular conditional and prototypical networks to the more niche latent space optimization methods, presenting also the new opportunities offered by recent foundational models. Through a chronological narrative, we dissect influential trends and methodologies, providing insights into their strengths and limitations. A temporal timeline offers a visual roadmap, marking key milestones in the field's progression. Complemented by quantitative analyses on benchmark datasets and qualitative showcases of seminal works, this survey equips readers with a deep understanding of the topic. By elucidating current challenges, state-of-the-art models, and prospects, we aid researchers and practitioners in navigating the intricacies of Few-Shot Semantic Segmentation and provide ground for future development.

==> 1shtoVSkshot.tex <==
\cite{BMVC2017_167} extend to k-shot by performing K prediction and using logical OR to enable the final results

==> abstract.tex <==
\section{Abstract}
Semantic segmentation, vital for applications ranging from autonomous driving to robotics, faces significant challenges in domains where collecting large annotated datasets is difficult or prohibitively expensive. In such contexts, such as medicine and agriculture, the scarcity of training images hampers progress.

Introducing Few-Shot Semantic Segmentation, a novel task in computer vision, aiming at designing models capable of segmenting new semantic classes with only a few examples. This paper embarks on a comprehensive survey of Few-Shot Semantic Segmentation, tracing its evolution and exploring various model designs, from the more popular conditional and prototypical networks to the more niche latent space optimization methods as well as presenting the more recent works based on foundational models.

Through a chronological narrative, we dissect influential trends and methodologies, providing insights into their strengths and limitations. A temporal timeline offers a visual roadmap, marking key milestones in the progression of the field.

Complemented by quantitative results on benchmark datasets and qualitative showcases of seminal works, this survey equips readers with a deep understanding of the topic. By elucidating current challenges, state-of-the-art models, and future prospects, we aim to aid researchers and practitioners in navigating the intricacies of Few-Shot Semantic Segmentation and provide ground for future development.

==> feature-comparison.tex <==
The authors of \cite{SG-ONE} found that the model based on a siamese design has the following weakneses:

1) The parameters of using the two parallel networks are redundant, which is prone to overfitting and leading to the waste of computational resources; 
2) combining the features of support and query images by mere multiplication is inadequate for guiding the query network to learn high-quality segmentation masks


-->

The authors of \cite{SG-ONE} proposes to extract the prototype vector of a class by applying the masked average pool on the support images, and then computing a similarity map as the cosine similarity between each feature vector and the prototype at each pixel location.

==> feature-extractor.tex <==
\cite{BMVC2017_167} uses VGG in the conditioning branch,  the FCN-32s fully convolutional architec-
ture \cite{Fully-conv-net} excluding the final prediction layer. 

==> masking.tex <==
In order to make the model learn to segment the subject labelled by the mask different approaches have been tried .

\cite{BMVC2017_167} decided to segment the subject in the images with its corresponding labels is a way to remove the background to from the image. This has been done according to the following reason:
(1) Even in the presence of the mask the network response tends to be biased towards the largest object in the image which may not be the object we would like to segment. 
(2) Including the background information in the input increased the variance of the output parameters {w, b} which prevented the network from converging.

==> transformers.tex <==
\cite{zhang2021few,zhang2019pyramid,wang2020few}


\cite{zhang2021few}
transformers self attention, then cross attention
